VIEW: Visual Imitation Learning with Waypoints

Robots can use Visual Imitation Learning (VIL) to learn manipulation tasks from video demonstrations. However, translating visual observations into actionable robot policies is challenging due to the high-dimensional nature of video data. This challenge is further exacerbated by the morphological differences between humans and robots, especially when the video demonstrations feature humans performing tasks. To address these problems we introduce Visual Imitation lEarning with Waypoints (VIEW), an algorithm that significantly enhances the sample efficiency of human-to-robot VIL. VIEW achieves this efficiency using a multi-pronged approach: extracting a condensed prior trajectory that captures the demonstrator's intent, employing an agent-agnostic reward function for feedback on the robot's actions, and utilizing an exploration algorithm that efficiently samples around waypoints in the extracted trajectory. VIEW also segments the human trajectory into grasp and task phases to further accelerate learning efficiency. Through comprehensive simulations and real-world experiments, VIEW demonstrates improved performance compared to current state-of-the-art VIL methods. VIEW enables robots to learn manipulation tasks involving multiple objects from arbitrarily long video demonstrations. Additionally, it can learn standard manipulation tasks such as pushing or moving objects from a single video demonstration in under 30 minutes, with fewer than 20 real-world rollouts. Code and videos here: https://collab.me.vt.edu/view/

==> algorithm.tex <==
\subsection{Algorithms}

\begin{algorithm}[]
\caption{Hand Trajectory Extraction}
\label{alg:hand_traj}
    \hspace*{\algorithmicindent} \textbf{Input:} Video of human interaction $V^h$ \\
    \hspace*{\algorithmicindent} Depth information $D^h$ \\
    \hspace*{\algorithmicindent} 100DOH hand detection model $100DOH$ \\
    \hspace*{\algorithmicindent} MANO analytical hand model  $MANO$ \\
    \hspace*{\algorithmicindent} Camera intrinsic and extrinsic parameters $\mathcal{C}^c_r$ \\
    \hspace*{\algorithmicindent} \textbf{Output:} Human hand trajectory $\xi^h$\\
    \begin{algorithmic}[1]
        \State Initialize $100DOH$, $MANO$
        \State Initialize an empty list $\xi^h$
        \For{Video frame $V^h_t$ in $V^h$}
            \State $p^x_t$, $p^y_t$, $c_t$ = \Call{$100DOH$}{$V^h_t$}
            \State $\delta^h_t$ = \Call{$D^h$}{$p^x_t$, $p^y_t$}
            \State $w^x_t$, $w^y_t$ = \Call{$MANO$}{$p^x_t, p^y_t$}
            \State $x^h_t, y^h_t, z^h_t$ = \Call{$\mathcal{C}^c_r$}{$w^x_t$, $w^y_t$, $\delta^h_t$}
            \State $w^h_i = \{x^h_t, y^h_t, z^h_t, c_t\}$
            \State Append $w^h_i$ to $\xi^h_i$
        \EndFor
    \end{algorithmic}
\end{algorithm}


\begin{algorithm}[]
\caption{Rewards}
\label{alg:reward}
    \hspace*{\algorithmicindent} \textbf{Input:} Video of robot interaction $V^r$ \\
    \hspace*{\algorithmicindent} object trajectory prior in pixels $\zeta^o_h$ \\
    \hspace*{\algorithmicindent} object tag $tag$ \\
    \hspace*{\algorithmicindent} \textbf{Output:} Reward for each waypoint $R$ \\
    \begin{algorithmic}[1]
        \State $\zeta^o_r$ = \Call{ExtractObjectTraj}{$V^r$, $tag$}
        \State Initialize an empty list $R$
        \For{$(p_{x_{t_i}}^r, p_{y_{t_i}}^r)$ in $\zeta^o_r$}
            \State Calculate $r_{t_i}$ using \eq{reward}
            \State Append $r_{t_i}$ to $R$
        \EndFor
        \State \Return R
    \end{algorithmic}
\end{algorithm}


\begin{algorithm}[]
\caption{Residual Learning}
\label{alg:reward}
    \hspace*{\algorithmicindent} \textbf{Input:} Dataset containing pairs of prior trajectories and the successful trajectories $\mathcal{D}(\xi, \xi^*)$
    \begin{algorithmic}[1]
        \State Randomly initialize the policy network $\pi$
        \For{iteration $i = 1, 2, \dots$}
            \State Sample a batch of $m$ waypoints $(\omega, \omega^*)$ from $\mathcal{D}(\xi, \xi^*)$
            \State Pass $\omega$ through the policy network to predict the correct waypoint $\hat{\omega}$
            \State Calculate the mean square loss with the true waypoint, i.e. $\mathcal{L} = \frac{1}{m} \sum_{j=1}^m (\omega^* - \hat{\omega})^2$
            \State Update the policy using the mean square loss
        \EndFor
    \end{algorithmic}
\end{algorithm}
